Joint Inference of Reward Machines and Policies for Reinforcement Learning

Incorporating high-level knowledge is an effective way to expedite reinforcement learning (RL), especially for complex tasks with sparse rewards. We investigate an RL problem where the high-level knowledge is in the form of reward machines, i.e., a type of Mealy machine that encodes the reward functions. We focus on a setting in which this knowledge is a priori not available to the learning agent. We develop an iterative algorithm that performs joint inference of reward machines and policies for RL (more specifically, q-learning). In each iteration, the algorithm maintains a hypothesis reward machine and a sample of RL episodes. It derives q-functions from the current hypothesis reward machine, and performs RL to update the q-functions. While performing RL, the algorithm updates the sample by adding RL episodes along which the obtained rewards are inconsistent with the rewards based on the current hypothesis reward machine. In the next iteration, the algorithm infers a new hypothesis reward machine from the updated sample. Based on an equivalence relationship we defined between states of reward machines, we transfer the q-functions between the hypothesis reward machines in consecutive iterations. We prove that the proposed algorithm converges almost surely to an optimal policy in the limit if a minimal reward machine can be inferred and the maximal length of each RL episode is sufficiently long. The experiments show that learning high-level knowledge in the form of reward machines can lead to fast convergence to optimal policies in RL, while standard RL methods such as q-learning and hierarchical RL methods fail to converge to optimal policies after a substantial number of training steps in many tasks.

==> alternative_example.tex <==
% !TEX root = main.tex

%\color{orange!90!black}

% \subsection{Alternative Motivating Example}

%As a motivating example, let us consider an autonomous vehicle whose task is to navigate in a residential area, as sketched in Figure~\ref{fig:ex:road-map}.
%As common in many European countries, some of the streets are priority streets.
%While traveling on a priority street, a car has the right-of-way and does not need to yield to traffic on intersections.
%Typically, priority roads start with a special sign and ends with a special sign. 
%(In reality, there might be different signs or conditions for an end of a priority road, but in this simple example we are abstracting that away.)
%In the example of Figure~\ref{fig:ex:road-map}, both roads going from west to east are priority roads (indicated by a gray shading), whereas the roads going from north to south are ordinary roads.
%
%\begin{figure}[th]
%	\centering
%	\begin{tikzpicture}
%		% Road
%		\draw[double=white, double distance=5mm, line width=.5mm] (0, 0) -- (6, 0) (0, -2) -- (6, -2) (2, 1) -- (2, -3) (4, 1) -- (4, -3);
%		\fill[gray!25] ([yshift=-2.5mm]0, 0) rectangle ([yshift=2.5mm]6, 0) ([yshift=-2.5mm]0, -2) rectangle ([yshift=2.5mm]6, -2);
%		
%		% Markings
%		\draw[dashed] (0, 0) -- (6, 0) (0, -2) -- (6, -2);
%		\draw[dashed] (2, 1) -- (2, .25) (4, 1) -- (4, .25) (2, -.25) -- (2, -1.75) (4, -.25) -- (4, -1.75) (2, -2.25) -- (2, -3) (4, -2.25) -- (4, -3);
%	
%		% Labels
%		\node[font=\bfseries] at (-.5, 0) {A};
%		\node[font=\bfseries] at (6.5, -2) {B};
%	
%	\end{tikzpicture}
%	
%	\caption{Map of a residential area} \label{fig:ex:road-map}
%\end{figure}
%
%
% \begin{figure}[b]
%		\centering                              
%		\includegraphics[width=9cm]{figures/traffic.pdf}                                         
%		\caption{\ZX{Map of a residential area}} \label{fig:ex:road-map}
%	\end{figure}   
%
%Let us assume that the task of the autonomous vehicle is to drive from position ``A'' (a start position) on the map to position ``B'' while obeying the traffic rules.
%To simplify matters, we are here only interested in the traffic rules concerning the right-of-way and how the vehicle acts at intersections.
%Moreover, we make the following two further simplifications: (1) we assume that the vehicle correctly senses the beginning and the end of a priority road (by recognizing the corresponding signs) and (2) we are only interested in whether or not the vehicle should yield to vehicles coming from the intersecting road (in a realistic scenario, the turning vehicle clearly also needs to consider opposing traffic).
%%other vehicles on its right side 
%
%Even for this simplified view, a memory-less policy does not suffice as the optimal action at any intersection depends on whether or not the vehicle is traveling on a priority road (which it might have entered multiple intersections before).
%More precisely, in our model, the vehicle is obeying the rules if and only if
%\begin{itemize}
%	\item it is traveling on a normal road, has traffic on the intersecting road, and yields to the traffic;
%	\item it is traveling on a normal road, has no traffic on the intersecting road, and does not yield; or
%	\item it is traveling on a priority road and does not yield (regardless of whether there is traffic on the intersecting road).
%\end{itemize}
%In particular, the vehicle violates the rules and does not get a reward if it yields on a priority road or on a normal road when there is no traffic on the intersecting road.
%
%An example reward machine for traveling on priority roads is shown in Figure~\ref{fig:ex:reward-machine}.
%Intuitively, state $p_0$ corresponds to the vehicle traveling on a normal road, while $p_1$ corresponds to the vehicle traveling on a priority road.
%While in $p_0$, the vehicle ends up in a sink state $p_x$ in case there is a traffic ($\mathit{tr}$) and it does not yield ($\lnot \mathit{y}$), or in case there is no traffic ($\lnot \mathit{tr}$) and it does yield ($\mathit{y}$). %; in both cases, the reward machine remains in state $p_0$.
%While in state $p_1$, on the other hand, the vehicle gets to the sink state if it yields, regardless of whether there is traffic on the right.
%The reward machine switches between states $p_0$ and $p_1$ on entering and exiting a priority road (indicated by $\mathit{pr}$ and $\lnot \mathit{pr}$, respectively).
%Finally, the reward 1 is obtained if from either $p_0$ or $p_1$ place $B$ is reached.
%
%
%\begin{figure}[th]
%	\centering
%	\begin{tikzpicture}
%		\node[state] (0) at (0, 0) {$p_0$};
%		\node[state] (1) at (3.5, 0) {$p_1$};
%		\node[state] (x) at (0, - 3.5) {$p_x$};
%		\node[state] (2) at (4.5, - 3.5) {$p_2$};
%		\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
%		\draw[->] (0) to[bend right] node[sloped, below, align=center] {$(\lnot B \land \mathit{tr} \land \lnot y, 0)$ \\ $(\lnot B \land \lnot \mathit{tr} \land y$,0)} (x);
%		\draw[->] (0) to[loop above] node[align=center] {$(\lnot B \land \lnot\textit{pr}, 0)$\\$(\lnot B \land \textit{tr} \land \mathit{y}, 0)$ \\ $(\lnot B \land \lnot\textit{tr} \land \lnot\mathit{y}, 0)$} ();
%		\draw[->] (0) to[bend right=10] node[sloped, above, align=center] {$(B, 1)$} (2);
%		\draw[->] (0) to[bend left=20] node {$(\lnot B \land \mathit{pr}, 0)$} (1);			
%		\draw[->] (1) to[loop above] node[align=center] {$(\lnot B \land \lnot\mathit{y}, 0)$ \\ $(\lnot B \land\mathit{pr}, 0)$} ();
%		\draw[->] (1) to[bend left] node [above]{$(\lnot B \land\lnot\mathit{pr}, 0)$} (0);
%		\draw[->] (1) to[bend left=20] node[align=left, sloped, below] {$(y,0)$} (x);
%		\draw[->] (1) to[bend left=10] node[align=center, sloped] {$(B, 1)$} (2);
%		\draw[->] (x) to[loop below] node {$(*,0)$} ();
%		\draw[->] (2) to[loop below] node {$(*,0)$} ();
%	\end{tikzpicture}	
%	\caption{Reward machine for traveling on priority roads} \label{fig:ex:reward-machine}
%\end{figure}
%
%
%\begin{figure}[th]
%	\centering
%	\begin{tikzpicture}
%	\node[state] (0) at (-0.5, 0) {$p_0$};
%	\node[state] (1) at (4.5, 0) {$p_1$};
%	\node[state] (2) at (4.5, 4.5) {$p_2$};
%	\node[state] (3) at (0, - 3.5) {$p_3$};
%	\node[state, accepting] (4) at (7, - 3.5) {$p_4$};
%	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
%	\draw[->] (0) to[left] node[above, align=center] {$(\lnot s \land \lnot\mathit{pr}, 0)$} (1);
%	\draw[->] (0) to[loop above] node[align=center] {$(\lnot s \land \mathit{pr}, 0)$} ();
%	\draw[->] (1) to[bend right] node[sloped, below, align=center] {$(s \land \lnot\mathit{pr}, 0)$} (2);
%	\draw[->] (2) to[bend right] node[sloped, below, align=center] {$(\lnot s \land \mathit{pr}, 0)$} (0);
%	\draw[->] (2) to[bend right] node[below, align=center] {$(s \land \lnot\mathit{pr}, 0)$} (3);
%	\draw[->] (0) to[bend right] node[below, align=center] {$(s \land \mathit{pr}, 0)$} (3);
%	\draw[->] (1) to[bend right] node[below, align=center] {$(\lnot s \land \mathit{pr}, 0)$} (3);
%	\draw[->] (1) to[bend left] node[above, align=center] {$(\lnot s \land \lnot\mathit{pr}, 0)$} (3);
%	\draw[->] (0) to[bend right] node[below, align=center] {$(B, 1)$} (4);
%	\draw[->] (1) to[bend left] node[below, align=center] {$(B, 1)$} (4);
%	\draw[->] (2) to[bend left] node[below, align=center] {$(B, 1)$} (4);
%	\draw[->] (2) to[bend right] node[below, align=center] {$(\lnot s \land \lnot\mathit{pr}, 0)$} (1);
%	\end{tikzpicture}	
%	\caption{\ZX{Revised Reward machine for traveling on priority roads. $s$: stop; $\lnot s$ not stop; $pr$: end in priority road; $\lnot pr$: end in normal road. Intiitively, $p_0$ is in priority road and $p_1$ is in normal road, $p_2$ is after stopping in normal roads (should stop for only one time unit, consecutive stopping also fails), $p_3$ fails and $p_4$ succeeds. }} \label{fig:ex:reward-machine}
%\end{figure}
%
%A corresponding labeled MDP is $\mdp = (\mdpStates, \mdpInit, \mdpActions, \mdpProb, \rmLabels, \rmLabelingFunction)$.
%A state $s \in \mdpStates$ is a quintuple $(x, y, \mathit{tr}, \mathit{pStart}, \mathit{pEnd})$.
%Coordinates $x$ and $y$ correspond to the physical location of the vehicle (on a discretized grid).
%Boolean variable $\mathit{tr}$ denotes whether there is a traffic from the right.
%Finally, Boolean variables $\mathit{pStart}$ and $\mathit{pEnd}$ denote whether a sign for a start (respectively, end) of the priority road is visible.
%
%The set of actions is $\mdpActions = \set{(0,1), (0,-1), (1,0), (-1,0), (0,0)}$, corresponding to going north, south, west, east and staying in place.
%The transition probability $\mdpProb$ is defined by 
%\[ 
%\mdpProb(s, a, s') = 
%\begin{cases}
%	0 &\neg (s \xrightarrow{a} s')\\
%	0.7 &s \xrightarrow{a} s' \land (s'.x, s'.y) \in \mathcal{J} \land s'.\mathit{tr} = \top \\
%	0.3 & s \xrightarrow{a} s' \land (s'.x, s'.y) \in \mathcal{J} \land s'.\mathit{tr} = \bot \\ 
%	0.5 &s \xrightarrow{a} s' \land (s'.x, s'.y) \not\in \mathcal{J}\\
%\end{cases}
%\]
%where $s \xrightarrow{a} s'$ defines possible transitions. 
%More precisely,  $s \xrightarrow{a} s'\equiv (s.x, s.y) + a = (s'.x, s'.y) \land s'.\mathit{pStart} \Leftrightarrow (s'.x, s'.y) \in \mathit{PriorityStart} \land s'.\mathit{pEnd} \Leftrightarrow (s'.x, s'.y) \in \mathit{PriorityEnd}$, where \textit{PriorityStart} and \textit{PriorityEnd} are sets of locations containing signs for start and end of priority road.
% The set of locations $\mathcal J$ represents an area for which there is expected increased traffic.
% Note that the randomness comes from the the actions of other cars, so the same action can bring the care into a state with traffic and the one without traffic.
%
%The set of labels is $\set{\mathit{tr}, \mathit{pr}, y, B}$ and the labeling function $\rmLabelingFunction$ is defined by
%\begin{align*}
%\mathit{tr} \in \rmLabelingFunction(s,a,s') &\Leftrightarrow s'.\mathit{tr} = \top \\
%\mathit{pr} \in \rmLabelingFunction(s,a,s') &\Leftrightarrow s'.\mathit{pStart} = \top \\
% &\lor(s.\mathit{pStart} = \top \land s'.\mathit{pEnd} = \bot )\\
%y \in \rmLabelingFunction(s,a,s') &\Leftrightarrow a = (0,0)\\
%B \in \rmLabelingFunction(s,a,s') &\Leftrightarrow s'.x = x_B \land s'.y = y_B
%\end{align*}

==> old_definitions.tex <==
\section{Appendix}

I have moved Zhe's definitions to the appendix. We will use them if needed.


\begin{definition}
	A weighted deterministic finite automaton (DFA) is a tuple $\mathcal{A}=(\mathcal{Q},q_{0},\Sigma,\delta,Acc, W)$ where
	$\mathcal{Q}=\{q_0, q_1, \dots, q_K\}$ is a finite set of states, $q_{0}$ is the initial state, $\Sigma$ is the alphabet, $\delta \colon \mathcal{Q}\times\Sigma\rightarrow\mathcal{Q}$ is the transition relation, $Acc\subseteq2^{\mathcal{Q}}$ is a finite set of accepting states, and $W: \mathcal{Q}\times\Sigma\times\mathcal{Q}\rightarrow\mathbb{R}$ is a transition weight function. 
	\label{DFA}
\end{definition} 

\begin{definition}
	A reward DFA is a weighted DFA $\mathcal{A}_{\textrm{r}}=(\mathcal{Q},q_{0},\Sigma,\delta, Acc, \mathcal{R})$,
	where $\mathcal{R}: \mathcal{Q}\times\Sigma\times\mathcal{Q}\rightarrow\mathbb{R}$ is a reward function. 
	\label{RM}
\end{definition} 

\begin{definition}
	A reward sequence generated from a state $q$ in a reward DFA $\mathcal{A}_{\textrm{r}}=(\mathcal{Q},q_{0},\Sigma,\delta,Acc, \mathcal{R})$ is a sequence $(\sigma_1, r_1),  (\sigma_2, r_2), \dots$,
	where there exist states $q^i\in\mathcal{Q}~(i=1,2,\dots)$ such that $r_1=\mathcal{R}(q,\sigma_1, q_1)$ and $r_i=\mathcal{R}(q_{i-1},\sigma_i, q_i)$ hold for for each $i\ge2$. 
	\label{reward_sequence}
\end{definition} 

\begin{definition}
	For two reward DFAs $\mathcal{A}_{\textrm{r}}^1=(\mathcal{Q}^1,q^1_{0},\Sigma^1,\delta^1, Acc^1, \mathcal{R}^1)$ and $\mathcal{A}_{\textrm{r}}^2=(\mathcal{Q}^2,q^2_{0},\Sigma^2,\delta^2, Acc^2, \mathcal{R}^2)$, a state $q^1\in\mathcal{Q}^1$ is \textit{equivalent} with a state $q^2\in\mathcal{Q}^2$ if and only if $\mathcal{L}_{\mathcal{A}_{\textrm{r}}^1}(q^1)=\mathcal{L}_{\mathcal{A}_{\textrm{r}}^2}(q^2)$, where $\mathcal{L}_{\mathcal{A}_{\textrm{r}}}(q)$ is the set of all possible reward sequences generated from $q$ in $\mathcal{A}_{\mathrm{r}}$. 
	\label{equ}
\end{definition} 

\begin{definition}
	A \textit{Markov decision process} (MDP) is defined by a tuple $\mathcal{P}= (S, S_0, A, P, \mathcal{AP},L)$, where $S=\{s^1,$ $s^2,\dots,s^H\}$ is a finite set of states, $S_0\subset S$ is the initial set of states, $A$ is a finite set of actions, $P \colon S\times A\times S\rightarrow[0,1]$ is a transition probability
	distribution, $\mathcal{AP}$ is a set of atomic predicates, and $L: S\rightarrow2^{\mathcal{AP}}$ is a labeling function.   
\end{definition} 

\begin{definition}[Reward Product MDP]
	Let $\mathcal{M}= (S, S_0, A, P, \mathcal{AP},L)$ be a MDP and $\mathcal{A}=(\mathcal{Q},q_0,2^{\mathcal{AP}},\delta,Acc, \mathcal{R})$ be a reward DFA. The reward product automaton $\mathcal{M}_{\mathrm{p}} \coloneqq \mathcal{M}\otimes\mathcal{A}=(S_{\mathrm{p}},S_{0\mathrm{p}},P^{\pi}_{\mathrm{p}}, Acc_{\mathrm{p}}, \mathcal{R}_{\mathrm{p}})$ is a tuple such that
	\begin{itemize}
		\item $S_{\mathrm{p}}=S\times\mathcal{Q}$ is a finite set of states;
		\item $S_{0\mathrm{p}}$ is the initial set of states where for each $s_{0\mathrm{p}}=(s^i,q)\in S_{0\mathrm{p}}$, $s^i \in S_0$, $q=\delta(q_0, L(s^i))$;	
		\item $P^{\pi}_{\mathrm{p}}((s,q),(s',q')) = \begin{cases}
		P^{\pi}(s,s') & \text{if } q'=\delta(q, L(s')); \\ 
		0 & \text{otherwise};
		\end{cases}$\\
		\item $Acc_{\rm{p}}=S\times Acc$ is a finite set of accepting states;\\
		\item $\mathcal{R}_{\mathrm{p}} \colon S\times\mathcal{Q}\times\Sigma\times S\times\mathcal{Q}\rightarrow\mathbb{R}$ is a function such that $\mathcal{R}_{\mathrm{p}}(s,q,a,s',q')=\mathcal{R}(q,a,q')$.
	\end{itemize}
\end{definition} 

	\begin{algorithm}[t]
	\caption{Transfer of Extended Q-functions.}                                                                                                                                                                    
	\label{policy}
	\begin{algorithmic}[1]
		\State \textbf{Inputs:}  $X^{\textrm{S}}$, $X^{\textrm{T}}$, $A$
		\State Initialize the policies
		\While{reward is below the threshold} 
        \State  Learn automaton $A$ that classifies $\tau^{+}$ and $\tau^{-}$   
        \State  Convert automaton to reward machine
        \State  Decompose the reward machine into equivalent submachines and assign a policy to each equivalent submachine               
		\EndWhile
		\State Return $\bar{Q}^{\textrm{T}}$  
	\end{algorithmic} 
\end{algorithm}      


